Essential minimum and obstruction degrees of translates of subtori

We study the obstruction degrees of translates of sub-tori of multiplicative tori and we show how they are connected to lower bounds for the essential minimum of these varieties. In particular, we combine our computations with results of A. Schinzel and of F. Amoroso - R. Dvornicich, that we thus extend to translates of sub-tori defined over CM fields. This shows that the essential minimum of these varieties have a geometric behavior similar to that of varieties which are not translates of sub-tori. We also refine and extend to translates of sub-tori a lower bound obtained by D. Bertrand in connexion with relations of multiplicative dependence of algebraic points. Finaly, we prove that in the functional case the conjectural lower bound for the essential minimum of sub-varieties of multiplicative tori is true and its proof is elementary.

==> macros.tex <==
% --- MACROS -----------------------------------------------------------

\catcode`\@=11
\newtoks\mataille\let\mataille\small
\def\@upprep{%
  \spaceskip1.3\fontdimen2\font plus1.3\fontdimen3\font}
\long\def\@xskipmath#1\(#2\){%
  \toks@\@xp\@xp\@xp{\@xp\the\@xp\toks@#1}%
  \@ifnotempty{#2}{\toks@\@xp{\the\toks@\(#2\)}\@xskipmath\@empty}}%
\def\@maketitle{\cleardoublepage\thispagestyle{copyright}
 \begingroup
 \uppercasenonmath\shorttitle
 \ifx\@empty\shortauthors \let\shortauthors\shorttitle
  \else \uppercasenonmath\shortauthors \andify\shortauthors \fi
  \toks@\@xp{\mataille\shortauthors}\@temptokena\@xp{\mataille\shorttitle}%
  \edef\@tempa{\@nx\markboth{\the\toks@}{\the\@temptokena}}\@tempa%
 \topskip\z@skip
 \vtop to 55 mm{%
 \parindent=0pt
 \hrule
 \medskip
 {\abstractfont\smf@journalhead\par}\vfil
 \begin{center}
 \def\baselinestretch{1.2}\large\vfil
   {\bfseries\smf@boldmath\MakeUppercase\@title\par}
 \vfil
   \ifx\@empty\smfbyname\else
     {\smfbyfont\smfbyname\ifsmf@byauthor\par\vfil\else\ \fi}%
   \fi
   {\edef\smfandname{{\noexpand\normalfont \smfandname}}
    \andify\authors\authors\par}
 \vfil \vrule height .4pt width .3\textwidth \vfil
 \end{center}}
 \@maketitlehook
 \par\bigskip
 \ifx\@empty\@dedicatory\else\@setdedicatory\medskip\fi
 \@setabstract\par\smallskip\@setaltabstract\par
 \bigskip\bigskip
 \endgroup}
\catcode`\@=12

%----- Paquets, format de page --------------------------------------

%\usepackage[english, french]{babel}  
\usepackage{smfthm}
%\usepackage{smfenum}
%\usepackage{amssymb}
%\usepackage{amscd}

%\usepackage{amssymb,amsmath,latexsym,epsfig,euscript}
\usepackage{pxfonts,textcomp}  

\addtolength{\hoffset}{-13mm} 
\addtolength{\textwidth}{26.1mm} 
\addtolength{\topmargin}{-17mm} 
\addtolength{\textheight}{36mm}

%----- Accents -----------------------------------------


\catcode`\@=11

\newdimen\f@ntdim
\def\ovg{\f@ntdim=\fontdimen6\font \font\f@nt=lasy10 at \f@ntdim
\ouvreg\f@nt\everypar={\ouvreg\f@nt}}
\def\og{\f@ntdim=\fontdimen6\font \font\f@nt=lasyb10 at \f@ntdim
\ouvreg\f@nt\everypar={\ouvreg\f@nt}}
\def\ouvreg#1{\leavevmode\hbox{#1\unskip\kern+0.20em(\kern-0.20em(\kern+0.20em}%
\ignorespaces\nobreak}

\def\fmg{\fermeg\f@nt\everypar={}} \let\fg=\fmg
\def\fermeg#1{\relax \ifhmode \unskip\kern+0.20em\else \leavevmode \fi%
\hbox{#1)\kern-0.20em)\kern+0.20em\ignorespaces}}

\catcode`\@=12 

\def\enoncesans#1#2 #3{\begin{thm}#1#3\end{thm}}
\def\enoncenormal#1#2 #3{\begin{prop}#1#3\end{prop}}
\def\cal#1{\mathcal{#1}}
\font\eightrm=ptmr at 8pt

\font\ninebf=cmbxti10 at 9pt
\font\sevenbf=cmbxti10 at 7pt

\font\fiverm=ptmr at 5pt
\def\^#1{\if#1i{\accent"5E\i}\else{\accent"5E #1}\fi} 
\def\"#1{\if#1i{\accent"7F\i}\else{\accent"7F #1}\fi} 
\catcode`\Ž=\active \def Ž{\'e}
\catcode`\ˆ=\active \def ˆ{\`a}
\catcode`\=\active \def {\`e}
\catcode`\=\active \def {\`u}
\catcode`\‰=\active \def ‰{\^a}
\catcode`\=\active \def {\^e}
\catcode`\"=\active \def "{\^\i}
\catcode`\™=\active \def ™{\^o}
\catcode`\ž=\active \def ž{\^u}
\catcode`\Š=\active \def Š{\"a}
\catcode`\'=\active \def '{\"e}
\catcode`\•=\active \def •{\"\i}
\catcode`\š=\active \def š{\"o}
\catcode`\Ÿ=\active \def Ÿ{\"u}
\catcode`\=\active \def {\c c}

\def\enmarged#1{\goodbreak\ifodd\count0\marginpar{\hbox{\ninebf#1\kern18mm}}
\else\marginpar{\hbox{\kern18mm\ninebf#1}}\fi}

\catcode`\é=\active \def é{\'e}
\catcode`\à=\active \def à{\`a}
\catcode`\è=\active \def è{\`e}
\catcode`\ù=\active \def ù{\`u}
\catcode`\â=\active \def â{\^a}
\catcode`\ê=\active \def ê{\^e}
\catcode`\î=\active \def î{\^\i}
\catcode`\ô=\active \def ô{\^o}
\catcode`\û=\active \def û{\^u}
\catcode`\ä=\active \def ä{\"a}
\catcode`\ë=\active \def ë{\"e}
\catcode`\ï=\active \def ï{\"\i}
\catcode`\ö=\active \def ö{\"o}
\catcode`\ü=\active \def ü{\"u}
\catcode`\ç=\active \def ç{\c{c}}

% -------------------- Comandos --------------------------------

\def\rank {{\rm \mbox{rank\,}}}
\def\Id {{\rm \mbox{Id}}}
\def\codim {{\rm \mbox{codim}}}

\def\Conv {{ \mbox{\rm Conv}}}
\def\conv {{ \mbox{\rm  \scriptsize Conv}}}
\def\Vol {{\mbox{\rm Vol}}}
\def\vol {\mbox{\rm vol\,}}
\def\ass {{\rm \mbox{Ass}}}

\def\Supp {{\mbox{\rm Supp}}}
\def\Hom {{\rm \mbox{Hom\,}}}
\def\ord {\mbox{\scriptsize ord}}
\def\Ord {\mbox{\rm ord}}
\def\GL {{\rm \mbox{GL}}}
\def\SL {{\rm \mbox{SL}}}

\def\dist {{\rm \mbox{dist}}}
\def\init {{\rm \mbox{init}}}
\def\initial {{\mbox{\scriptsize \rm init}}}
\def\Res {\mbox{\rm R{\'e}s}}
\def\aff {{\rm \mbox{\scriptsize aff}}}

\def\sat {{\rm \mbox{\scriptsize sat}}}
\def\Adj { \mbox{\rm Adj}}
\def\Diag { \mbox{\rm Diag}}
\def\discr {\mbox{\rm discr}}

\def\mmax {{\mbox{\rm \scriptsize max}}}
\def\h {{ \mbox{\rm \scriptsize h}}}
\def\red {{ \mbox{\rm \scriptsize red}}}
\def\gal {{ \mbox{\rm \scriptsize Gal}}}
\def\Gal {\mbox{\rm Gal}}

\def\Rang {\mbox{\rm Rang\,}}
\def\ess {{ \mbox{\rm \scriptsize ess}}}
\def\abs {{ \mbox{\rm \scriptsize abs}}}
\def\m {{ \mbox{\rm \scriptsize m}}}

\newcommand{\ab}{{\rm ab}}
\def\cc {{ \mbox{\rm \scriptsize c}}}
\def\ccc {{ \mbox{\rm \tiny c}}}

\def\pr {{ \mbox{\rm \scriptsize pr}}}
\def\ssup {{ \mbox{\rm \scriptsize sup}}}
\def\span {\mbox{\rm span}}
\def\covol {\mbox{\rm covol}}

\def\im {\mbox{\rm Im}\,}
\def\Div {\mbox{\rm Div}}
\def\div {\mbox{\rm div}}
\def\Tors {\mbox{\rm Tors}}
\def\tors {{ \mbox{\rm \scriptsize tors}}}

\def\Ann {\mbox{\rm Ann}}
\def\reg {\mbox{\rm reg}}
\def\graph {\mbox{\rm graph}}
\def\Hess {\mbox{\rm Hess}}

\def\lg {\mbox{\rm lg}}
\def\Ass {\mbox{\rm \scriptsize Ass}}
\def\Irr {\mbox{\rm Irr}}
\def\irr {\mbox{\rm \scriptsize Irr}}
\def\FS {\mbox{\rm \scriptsize FS}\,}
 
\def\proj {{\mbox{\rm \scriptsize proj}}}
\def\weyl {{\mbox{\rm \scriptsize W}}}
\def\laurent {{\mbox{\rm \scriptsize Lau}}}
\def\daph {{\mbox{\rm \scriptsize DP}}}

\def\geom {{\mbox{\rm \scriptsize g{\'e}om}}}
\def\norm {{\mbox{\rm \scriptsize norm}}}
\def\arith {{\mbox{\rm \scriptsize arith}}}

\def\Spec   {\mbox{\rm Spec}\,}
\def\MV {\mbox{\rm MV}}
\def\MI {\mbox{\rm MI}}
\def\NP {\mbox{\rm N}}
\def\adeg {\wh{\deg}}

\def\Card {\mbox{\rm Card}}
\def\card {{\mbox{\rm \scriptsize Card}}}
\def\Ch {{\mathcal{C}{\it h}}}
\def\Aff {\mbox{\rm Aff}}

\def\diag {\mbox{\rm diag}}
\def\Mat {\mbox{\rm Mat}}
\def\Expo {\mbox{\rm Expo}}
\def\expo {\mbox{\rm \scriptsize Expo}}
\def\Ker {\mbox{\rm Ker}}

\def\Spec {\mbox{\rm Spec}}
\def\DPC  {\mbox{\rm DPC}}
\def\dpc  {\mbox{\rm \scriptsize DPC}}
\def\Pan  {\mbox{\rm Pan}}
\def\pan  {\mbox{\rm \scriptsize Pan}}
\def\longueur  {\mbox{\rm long}}

\def\OK {{\cO_K}}
\def\Hnorm {\mathcal{H}_\norm}
\def\Harith {{\mathcal{H}_\arith}}
\def\hnorm {{\widehat{h}}}
\def\munorm {{\widehat{\mu}}}

\def\geom {{\mathcal A}}
\def\arith {{{\mathcal A}, \alpha}}

\def\Faces {{\mbox{\rm F}}}
\def\faces {{\mbox{\rm \scriptsize F}}}
\def\res {\mbox{\rm r{\'e}s}}
\def\Newton {\mbox{\rm N}}

\def\ov#1{{\overline{#1}}}
\def\un#1{{\underline{#1}}}
\def\wh#1{{\widehat{#1}}}
\def\wt#1{{\widetilde{#1}}}

\newcommand{\mug}{\mbox{\boldmath{$\muup$}}}
\newcommand{\Gammag}{\mbox{\boldmath{$\Gamma$}}}

% -------------------- Letras Especiales -------------------------

\def \k {{\bf k}}
\def \t {{\bf t}}
\def \w {{\bf w}}
\def \x {{\bf x}}

\def \A {{\bf A}}
\def \C {{\bf C}}
\def \G {{\bf G}}
\def \N {{\bf N}}
\def \P {{\bf P}}
\def \Q {{\bf Q}}
\def \R {{\bf R}}
\def \Z {{\bf Z}}

\def \cA {\mathcal{A}}
\def \cB {\mathcal{B}}
\def \cC {\mathcal{C}}
\def \cD {\mathcal{D}}
\def \cE {\mathcal{E}}
\def \cF {\mathcal{F}}
\def \cG {\mathcal{G}}
\def \cH {\mathcal{H}}
\def \cI {\mathcal{I}}
\def \cJ {\mathcal{J}}
\def \cK {\mathcal{K}}
\def \cL {\mathcal{L}}
\def \cM {\mathcal{M}}
\def \cN {\mathcal{N}}
\def \cO {\mathcal{O}}
\def \cP {\mathcal{P}}
\def \cQ {\mathcal{Q}}
\def \cR {\mathcal{R}}
\def \cS {\mathcal{S}}
\def \cT {\mathcal{T}}
\def \cU {\mathcal{U}}
\def \cV {\mathcal{V}}
\def \cW {\mathcal{W}}
\def \cX {\mathcal{X}}
\def \cY {\mathcal{Y}}
\def \cZ {\mathcal{Z}}

\def\ga {{\mathfrak{a}}}
\def\gf {{\mathfrak{f}}}
\def\gothg {{\mathfrak{g}}}
\def\gp {{\mathfrak{p}}}
\def\gq {{\mathfrak{q}}}
\def\gM {{\mathfrak{M}}}

\def\cad {c'est-à-dire } 
\def\spdg {sans perte de généralité }

\def\Qbar {{\overline{\Q}}}
\def\h{{\widehat{h}}}
\def\kbar {{\overline{k}}}

%---
\newcommand{\declare}[1]{\refstepcounter{x}{c_{\thex}\label{#1}}}
\newcommand{\use}[1]{{c_{\ref{#1}}}}
\newcounter{x}

\font\bmath=cmmib10

\font\danger=pzcmi at 48pt
\def\enmarge#1{\goodbreak\relax\marginpar{\ifodd\count0
\vtop{\hsize=1.8cm\vskip-0.2cm\danger Z\par{\bf #1}}\else
\vtop{\hsize=3.3cm\vskip0cm\leftskip1.4cm\danger Z\par{\bf #1}}\fi}\nobreak}

\font\grossc=cmcsc10 at 10pt

\endinput



